Touch the Core: Exploring Task Dependence Among Hybrid Targets for Recommendation

As user behaviors become complicated on business platforms, online recommendations focus more on how to touch the core conversions, which are highly related to the interests of platforms. These core conversions are usually continuous targets, such as \textit{watch time}, \textit{revenue}, and so on, whose predictions can be enhanced by previous discrete conversion actions. Therefore, multi-task learning (MTL) can be adopted as the paradigm to learn these hybrid targets. However, existing works mainly emphasize investigating the sequential dependence among discrete conversion actions, which neglects the complexity of dependence between discrete conversions and the final continuous conversion. Moreover, simultaneously optimizing hybrid tasks with stronger task dependence will suffer from volatile issues where the core regression task might have a larger influence on other tasks. In this paper, we study the MTL problem with hybrid targets for the first time and propose the model named Hybrid Targets Learning Network (HTLNet) to explore task dependence and enhance optimization. Specifically, we introduce label embedding for each task to explicitly transfer the label information among these tasks, which can effectively explore logical task dependence. We also further design the gradient adjustment regime between the final regression task and other classification tasks to enhance the optimization. Extensive experiments on two offline public datasets and one real-world industrial dataset are conducted to validate the effectiveness of HTLNet. Moreover, online A/B tests on the financial recommender system also show that our model has improved significantly. Our implementation is available here\footnote{\url{https://github.com/fuyuanlyu/HTLNet}}.

==> section/rebuttal.tex <==
To all reviewers:
Thanks for your careful and thorough reading of this paper and your thoughtful comments and constructive suggestions, which are very helpful in improving its quality. The list below explains in detail our responses to the Reviewers’ comments, including some general and individual questions, which we hope will help the reviewers re-evaluate our paper.

[GQ1: Some typos and presentation issue (R1,R2,R3,R4)]
We have revised these issues based on the reviewers' comments. We have also made some other necessary revisions and gone through the whole manuscript several times to polish its presentation.

[GQ2: Why gumbel-softmax is adopted here? (R2,R3，R4)]
Actually, there are some alternatives to enable label transfer. First, we can use the golden labels of all the low-level tasks to utilize the discrete labels during the training stage,. However, the golden label is unavailable in the test stage, which leads to train-test discrepancy. To overcome this issue, we can sample a label from the predicted probability. Notice that the sample operation is not differentiable. 
Specifically, the embedding corresponding to the sampled label will be the only one updated in the backpropagation. This will lead to high-variance gradients making the optimization unstable. Moreover, the low-level task will have a certain probability of sampling a counterfactual value, and get feedback from high-level tasks if there is relation exists. As a result, we introduce the Gumbel-softmax operation, which uses a re-parameter trick with a temperature to approximate sampling.


[GQ3: Intuition behind the optimization strategy (R3,R4)]
One of the challenges in our work is training the proposed HTLNet more efficiently and effectively with the hybrid targets. As discussed in the paper, the gradients differ greatly in hybrid targets, and the influence of core targets on other tasks is large. 
We propose a customized optimization strategy for our HTLNet based on previous research. Firstly, we carefully design the backpropagation mechanism. Then, shared embedding is the only factor that influences all the tasks. We hypothesize the vital factor is the unmatched gradients between the core target and preceding tasks. In our optimization, we first make two gradients in the same direction, corresponding to Equation 16. After resolving the direction conflict, we make the two gradients of the same magnitude, corresponding to Equation 17. The experimental results in Figure 6 suggest that the hypothesis holds. Therefore, the customized optimization strategy differs with previous study which is essential in our model.

*******************************************************
Reviewer 1:
We appreciate your suggestion. We will carefully check the full text and revise the manuscripts to enhance clarity. 

[W2: Reason for adopting different metrics] 
In KuaiRand, the core target is watch time, while in Kaggle-Revenue, it is the number of repurchases in one month. These targets are continuous, and NRMSE and NMAE are widely adopted to measure them. However, for revenue, spearman and Gini are used to measure the rank, which is also crucial in Lifetime value prediction.

[W3: Efficiency analysis]
We will add results on efficiency in the appendix of the revised version.

*******************************************************
Reviewer 2:
We thank you for your detailed suggestion. We will revise the paper according to your detailed comments.

[W1: Reproducbility] 
Once accepted, we will open-source the code. As you suggested, an open-source product dataset is helpful. Hence, we will conduct the necessary applications and checks within the company to ensure the dataset is open to the research community.

[W2: Limitations and future work]
Thanks for proposing this point. We will add more discussion in the conclusion in the following revision.

[P1:The motivation for introducing the Gumbel-softmax operation]
Please kindly refer to the GQ2.

[P2: Investigating different time slots]
Different time slots are worth investigating to enhance the robustness. However, most previous works used these datasets divided datasets in chronological order to avoid leakage from the timeline[1,2]. So, we adopt a similar data processing here.
[1]. Ziru Liu, et.al. 2023. Multi-Task Recommendations with Reinforcement Learning. In Proceedings of the ACM Web Conference 2023 (WWW '23).
[2].Haiyuan Zhao, et.al. 2023. Uncovering User Interest from Biased and Noised Watch Time in Video Recommendation. In Proceedings of the 17th ACM Conference on Recommender Systems (RecSys '23). 

[P3: Statistical Evaluation in Table 4,5,6] 
We are sorry to miss the statistical tests in Tables 4,5,6. Regarding these experiments which are mainly ablation or analysis of HTLNet, we ignore the tests. We will add these in the revision.

[P4: Regarding Figures 5 and 7] 
In Figure 5, we investigate the effect of different operations in IFU. Notice that the inputs to the operation are the label embedding and task representation from all the preceding tasks, the operation indicates how to fuse these information. As the results in Figure 5 indicate, the attention mechanism performs better than concatenation overall. The performance of classification tasks suffers a drop with concatenation operation because directly fusing information from a preceding task cannot avoid the negative transfer. The first one, click prediction, also performs better with attention, indicating that transferring inappropriate information will influence preceding tasks with shared embedding. As to the core target, the attention mechanism can adaptively learn what and how much information to transfer from preceding tasks.
In Figure 7, we conduct the online experiments. On most days, our HTLNet performs better than the baseline. As to different targets, both click and purchase behaviors perform consistently well. However, the purchase amount is considered more fluctuant due to the difficulties in the regression target, which further emphasizes our study.
We will further enhance the analysis accordingly in our revision.

*******************************************************
Reviewer 3:
We thank you for your kind reviews and appreciate our efforts in modeling task dependence among hybrid targets.

[W1: The motivation explained why Gumbel-softmax operation and the hyperparameters effect.]
Regarding the motivation for gumbel-softmax, kindly refer to the explanation in GQ2, as multiple reviewers have this question.
Regarding how the hyper-parameter affects the performance, the temperature tau controls the convergence speed of the model. Gumbel-Softmax approximates the unit-step function. In our setting, it is initialized as 10 and gradually decreases by 0.5x each N step. A faster-decreasing speed of tau generally makes the model converge faster. We will add this hyperparameter sensitivity in Appendix A.4.

[W2: The intuitive and explanation of Optimization Strategy]
Please kindly refer to the GQ3.

[W3: Details from model complexity perspective] 
Due to space limitations, we moved the concrete arch design for experiments to the appendix; please refer to it. To enhance reproducibility, we will open-source the code upon acceptance, which will give more details.

*******************************************************
Reviewer 4:
We thank you for your kind reviews and your professional comments on optimization.

[W1: Missing Existing Methods] 
Please allow us to highlight the motivation of our papers here, as our writings may not be optimal and can confuse the reviewer. 
Most previous works have already focused on multi-task learning for recommendation. Our work focuses more on sequential dependence, which also involves hybrid targets. As Reviewer 3 mentioned, this task is less frequently discussed but is a common situation in the industry. As in your professional comments, some problems have been discussed more or less in previous MTL works. For example, AITM is architecture for sequential tasks, and MetaBalance is an optimization strategy for MTL. 
However, we must emphasize that the hybrid targets introduce more challenges to these existing works. We identify two challenges in our work: (i) how to explore the dependence among hybrid targets and (ii) how to optimize the complex model. Specifically, the dependence from the classification task to the core regression task is complicated to model, which motivates us to propose label embedding and introduce LEU and IFU to fuse the relevant information. Because of hybrid targets, the gradient to optimize the model differs significantly between the preceding and core tasks; thus, we propose an optimization strategy to resolve the issue. All of these efforts are made to resolve the issues in task dependence modeling among hybrid targets. 

Therefore, simple mixed-together approaches are difficult to work well on our problem. We compare our HTLNet with three categories of methods: simple MTL, SDMTL, and optimization strategy. Moreover, we have also conducted an ablation study on our main component in Table 4 and analyzed both architecture and optimization in Table 5 and Table 6, respectively. Notice that simply replacing our optimization with Metabalance will decrease performance, further verifying our careful HTLNet design.
Nevertheless, we honestly admit that the lack of open-sourced datasets is a challenge in our experiments. As mentioned in MetaBalance, the Alibaba dataset is the appropriate choice for multitask learning for recommendation. It consists of three behaviors: buy, add-to-cart, and add-to-favorite. We did not choose this dataset mainly because of two reasons. First, the behavior is not sequence dependent, i.e., buy will not depend on add-to-cart or add-to-favorite; besides, add-to-cart and add-to-favorite are two separate behavior. In KuaiRand, the long view will depend whether user clicks the video, and the watch time is the core continuous target dependent on the long view. Second, there are no hybrid targets; all three behaviors fall into the single target, 0/1. 
In all, we do not choose this dataset in our experimental settings. And we will open source our private dataset when necessary checks by company are completed.

[W2: Presentation Issue] 
Thank you for pointing out our presentation issue. We discuss the optimization method in the introduction. Your professional comment reminds us of the balance between the introduction and related work and the completeness of the discussion on related work. We will discuss and cite the related works you mentioned in our revision. As mentioned, despite previous work addressing problems of task magnitudes and task relationships, exploring the dependence among hybrid tasks is outside these abilities.

[W3: Regarding Number of Tasks] 
Thank you for your constructive comments. Scaling with the increase in the number of tasks is an important indicator. To be honest, we have tried our best to find appropriate open-source datasets in our experiments. Unfortunately, few datasets satisfy our problem settings. We have conducted an experiment in our private targeted display advertising scenario which includes more tasks: exposure, click, application, approval, activation, and revenue. We will give detailed results as soon as possible in our revision.

[Q1: Regarding Gumbel-softmax] 
The motivation of Gumbel-softmax please refer to GQ2. Although the gradients will not be propagated into the task towers in our optimization, the optimization of label embedding is also crucial. With the Gumbel-softmax operation, both the label embeddings will be updated during the convergence, and the output becomes a one-hot vector as converges finally. While if the operation is not discrete, the sampled embedding is the sole one to update, which will introduce the unstable gradients in the optimization with independent sampling. 


*******************************************************
We thank all reviewers for pointing out our flaws. Hopefully, our reply can address their concerns. We believe all revision points can be fixed. We will revise the manuscripts accordingly.


==> section/rebuttal_x.tex <==
To all reviewers:
Thanks for your careful and thorough reading of this paper and your thoughtful comments and constructive suggestions, which are very helpful in improving its quality. The list below explains in detail our responses to your comments, including some general and individual questions, which we hope will help the reviewers reevaluate our paper.

[GQ1: Some typos and presentation issue (R1, R2, R3, R4)]
We have revised these issues based on the reviewers' comments. We have also made other necessary revisions and reviewed the whole manuscript several times to polish its presentation.

[GQ2: Why gumbel-softmax is adopted here? (R2, R3, R4)]
A straightforward strategy is to use the true labels of all predecessor tasks for label transfer. However, since the true labels are available during training but not during testing, this leads to the training-test discrepancy problem.
To this end, we select proxy labels from the predicted probabilities of the predecessor tasks for label transfer. Simple sampling operations are detrimental to model training because they are non-differentiable. On the one hand, only the label embedding corresponding to one sampled category is updated. This one-sided update quickly leads to high variance in the gradients between different label embeddings and makes the optimization unstable. On the other hand, label transfer based only on information from one category label may be insufficient, especially when the labels of the underlying task are noisy.
To alleviate these problems, we introduce gumbel-softmax to perform a differentiable sampling operation. This means that the model can use the information of all category labels in the early stage to perform inference in label transfer and update the label embeddings of all categories simultaneously. Then, as training progresses, the model gradually and smoothly converges to the final proxy labels and corresponding label embeddings.

[GQ3: Intuition behind the optimization strategy (R3, R4)]
The optimization of HTLNet needs to consider the significant impact of the core target on other tasks in backpropagation, as well as the inconsistent properties of the (continuous) core target and (category) other targets relative to the gradient.
As described in Section 4.2, the core target impacts other tasks mainly through shared embeddings and transferred information. For ease of processing, we first revise the backpropagation mechanism to make shared embeddings the only influencing factor (i.e., Eq. (15)).
We then assume that gradients' inconsistent properties can be quantified in terms of both direction and magnitude. We handle the direction conflict of their gradients on the shared embedding through Equation 16 and encourage their gradients to have similar magnitudes through Equation 17.
The experimental results in Figure 6 demonstrate that this assumption holds. Therefore, the customized optimization strategy differs from previous studies, which is crucial for our model.

*******************************************************
To Reviewer 1:
[W2: Reason for adopting different metrics] 
The core target of KuaiRand is the watch time, while the core targets of Kaggle-Revenue and products involve the amount. Since these targets are continuous, NRMSE and NMAE are commonly used indicators to measure them. Due to the particularity of the amount, Spearman and Gini are usually used to measure the ranking of predictions in industrial applications. Therefore, the latter two datasets will include more metrics. We will add more descriptions in the revised version.

[W3: Efficiency analysis]
We will add results on efficiency in the appendix of the revised version.

*******************************************************
To Reviewer 2:
[W1: Reproducbility] 
Once the paper is accepted, we will make the source code public. We agree with you that open-source product datasets are helpful. Hence, we will conduct the necessary applications and checks within the company to ensure the dataset is open to the research community.

[W2: Limitations and future work]
Thanks for your valuable comment! We will add more discussion in the conclusion in the revised revision.

[Q1: The motivation for introducing the Gumbel-softmax operation]
Please kindly refer to the GQ2. We will add more description and discussion in the revised version.

[Q2: Investigating different time slots]
Thanks for your valuable comment! We agree that different time slots are worth studying to verify the proposed method's robustness further. We will conduct additional experiments in this regard.

[Q3: Statistical Evaluation in Table 4,5,6] 
We apologize for missing the statistical tests in Tables 4, 5, and 6. Considering that these experiments involve analyzing HTLNet rather than comparing it with existing baselines, we previously ignored them. We will add them in the revised version.

[Q4: Regarding Figures 5 and 7] 
In Figure 5, we investigate the effect of different operations in IFU. Notice that the inputs to the operation are the label embedding and task representation from all the preceding tasks, and the operation indicates how to fuse this information. As the results in Figure 5 indicate, the attention mechanism performs better than concatenation overall. The performance of classification tasks suffers a drop with concatenation operation because directly fusing information from a preceding task cannot avoid the negative transfer. The first one, click prediction, also performs better with attention, indicating that transferring inappropriate information will influence preceding tasks with shared embedding. As to the core target, the attention mechanism can adaptively learn what and how much information to transfer from preceding tasks.
In Figure 7, we conduct the online experiments. On most days, our HTLNet performs better than the baseline. As to different targets, both click and purchase behaviors perform consistently well. However, the purchase amount is considered more fluctuant due to the difficulties in the regression target, which further emphasizes our study.
We will further enhance the analysis accordingly in our revision.

*******************************************************
To Reviewer 3:
[W1: The motivation explained why gumbel-softmax operation and the hyperparameters effect.]
Regarding the motivation for gumbel-softmax, please refer to the GQ2.
Regarding how the hyperparameter affects performance, the temperature tau controls the model's convergence speed. Gumbel-Softmax approximates the unit-step function. In our setting, it is initialized as 10 and gradually decreases by 0.5x each N step. A faster-decreasing speed of tau generally makes the model converge faster. We will add this hyperparameter sensitivity in Appendix A.4.

[W2: The intuitive and explanation of Optimization Strategy]
Please kindly refer to the GQ3.

[W3: Details from model complexity perspective] 
Due to space limitations, we moved the concrete arch design for experiments to the appendix; please refer to it. To enhance reproducibility, we will open-source the code upon acceptance, which will give more details.

*******************************************************
Reviewer 4:
[W1: Missing Existing Methods] 
We apologize for confusing you about our motivation and goal, which may be due to our unclear writing.
Please allow us first to emphasize the motivation and goal of our paper here: Most previous works have already focused on multi-task learning for recommendation, and each task target is usually categorical. Our work highlights hybrid targets' importance and unique challenges, where the core target differs from previous works and has continuous properties. As mentioned by Reviewer 3, this task is less frequently discussed but is a common situation in the industry. 
As mentioned in your professional review, some problems have been discussed more or less in previous MTL works. For example, AITM is architecture for sequential tasks, and MetaBalance is an optimization strategy for MTL. However, as described in the paper, hybrid targets bring more specific challenges to these existing works: (i) how to explore the dependence among hybrid targets and (ii) how to optimize the complex model. Specifically, the dependence from the classification task to the core regression task is complicated to model, which motivates us to propose label embedding and introduce LEU and IFU to fuse the relevant information. Because of hybrid targets, the gradient to optimize the model differs significantly between the preceding and core tasks; thus, we propose an optimization strategy to resolve the issue. All of these efforts are made to resolve the issues in task dependence modeling among hybrid targets. 
Therefore, simple mixed-together approaches are difficult to work well on our problem and our work should not be simply viewed as a hybrid setting of previous works. We compare our HTLNet with three categories of methods: simple MTL, SDMTL, and optimization strategy. Moreover, we have also conducted an ablation study on our main component in Table 4 and analyzed both architecture and optimization in Table 5 and Table 6, respectively. In particular, as shown in Table 6, simply replacing our optimization with Metabalance will decrease performance, further verifying our careful HTLNet design.

Nevertheless, we honestly admit that the lack of open-sourced datasets is a challenge in our experiments. As mentioned in MetaBalance, the Alibaba dataset is the appropriate choice for multitask learning for recommendation. It consists of three behaviors: buy, add-to-cart, and add-to-favorite. We did not choose this dataset mainly because of two reasons. First, the behavior is not sequence dependent, i.e., buy will not depend on add-to-cart or add-to-favorite; besides, add-to-cart and add-to-favorite are two separate behavior. As a counterexample, in KuaiRand, the long view will depend on whether the user clicks the video, and the watch time is the core continuous target dependent on the long view. Second, there are no hybrid targets; all three behaviors fall into the single target, 0/1, which does not fit our motivation and goals.
Therefore, we do not choose this dataset in our experimental settings. Other MTL datasets face similar limitations. We will open-source our private dataset when the company has completed the necessary checks.

[W2: Presentation Issue] 
Thank you for pointing out our presentation issue. We discuss the optimization method in the introduction. Your professional comment reminds us of the balance between the introduction and related work and the completeness of the discussion on related work. We will discuss and cite the paper you mentioned in our revision. As mentioned, despite previous work addressing problems of task magnitudes and task relationships, exploring the dependence among hybrid tasks is outside these abilities.

[W3: Regarding Number of Tasks] 
Thank you for your constructive comments. We agree that scalability as the number of tasks increases is an important metric. We have tried our best to find suitable open-source datasets in our experiments. Unfortunately, few datasets (including those with different numbers of tasks) meet our problem setting. To supplement this issue, we conducted experiments in the private targeted display advertising scenario, which includes more tasks: exposure, click, application, approval, activation, and revenue, and the preliminary experimental results have similar conclusions to those in the paper. We will give detailed results in the revised version.

[Q1: Regarding Gumbel-softmax] 
Regarding the motivation for gumbel-softmax, please refer to the GQ2. 
We want to emphasize that although gradients are not propagated to the task tower in our optimization, it is also crucial for optimizing label embeddings. With the gumbel-softmax operation, all label information is fully considered in the label transfer and both label embeddings are updated during the convergence process. As training progresses, the output of gumbel-softmax gradually converges to a one-hot vector in a gentle form. If the sampling operation is directly adopted, the sampled category embedding is the only updated embedding, which widens the difference between different category embeddings. Such a one-sided update is prone to introduce unstable gradients in model optimization.

*******************************************************

Again, we thank all reviewers for pointing out the flaws in this current version. We hope that our responses address your primary concerns. We believe all points can be fixed and will revise the manuscripts accordingly.


==> tables/table_main.tex <==

% \begin{table*}[htbp]
% \caption{Results on two public datasets, where the best and second best results are marked in bold and underlined, respectively. Each experiment is repeated 10 times for statistical confidence, and $^{*}$ indicates a significance level of $p\leq 0.05$ based on a two-sample t-test between our method and the best baseline.}
% \centering
% \scalebox{1.0}{
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|cc|cc|cc|cc|cc|cccc}
% \specialrule{0.1em}{3pt}{3pt}
%  {Dataset} & \multicolumn{6}{c|}{KuaiRand} & \multicolumn{8}{c}{Kaggle-Revenue} \\
%  \specialrule{0.05em}{1pt}{1pt}
%     {Task} & \multicolumn{2}{c|}{click} & \multicolumn{2}{c|}{long view} & \multicolumn{2}{c|}{watch time} & \multicolumn{2}{c|}{repurchase 1Y} & \multicolumn{2}{c|}{repurchase 1M}& \multicolumn{4}{c}{repurchase 1M amt} \\
    
%     Metrics & AUC$\uparrow$ & LogLoss$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & NRMSE$\downarrow$ & NMAE$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & NRMSE$\downarrow$ & NMAE$\downarrow$ & Spearman$\uparrow$ & Gini$\uparrow$ \\ 
    
%     \specialrule{0.05em}{2pt}{2pt}
    
%     DNN & 0.7512 & 0.4074 & 0.7698 & 0.2536 & 0.8979 & 0.9553 & 0.6892 & 0.3830 & 0.6255 & 0.6542 & 0.9985 & 1.0902 & 0.2339 & 0.5093 \\ 
%     Share Bottom & 0.7399 & 0.4115 & 0.7685 & 0.2543 & 0.8968 & 0.9620 & 0.6568 & 0.3931 & 0.6134 & 0.6606 & 0.9984 & 1.1064 & 0.2340 & 0.5090 \\ 
%     MMoE & 0.7379 & 0.4127 & 0.7645 & 0.2566 & 0.8970 & 0.9621 & 0.6696 & 0.3903 & 0.6161 & 0.6593 & 0.9987 & \underline{1.0623} & 0.2357 & 0.5093 \\ 
%     PLE & 0.7409 & 0.4110 & 0.7694 & 0.2542 & \underline{0.8963} & 0.9648 & 0.6732 & 0.3885 & 0.6178 & 0.6598 & 0.9988 & 1.0708 & 0.2332 & 0.5136 \\
%     AdaTT & 0.7396 & 0.4120 & 0.7683 & 0.2550 & 0.8975 & \underline{0.9508} & 0.6720 & 0.3888 & 0.6187 & 0.6580 & 0.9987 & 1.0969 & \underline{0.2419} & \underline{0.5185} \\ 
%     ESMM & 0.7303 & 0.4259 & 0.7540 & 0.2832 & 0.8981 & 0.9605 & 0.6361 & 0.6871 & 0.6046 & 0.7755 & 0.9989 & 1.1981 & 0.2379 & 0.5131 \\ 
%     AITM & 0.7391 & 0.4118 & 0.7672 & 0.2552 & 0.8978 & 0.9533 & 0.6728 & 0.3871 & 0.6151 & 0.6579 & \underline{0.9982} & 1.1274 & 0.2204 & 0.5029 \\ 
%     MetaBalance & \underline{0.7541} & \underline{0.4065} & \underline{0.7768} & \underline{0.2527} & 0.8967 & 0.9509 & \underline{0.6896} & \underline{0.3825} & \underline{0.6267} & \underline{0.6539} & 0.9985 & 1.1265 & 0.2376 & 0.5100 \\ 
%     \specialrule{0.05em}{1pt}{1pt}
%     HTLNet & $\textbf{0.7574}^{*}$ & $\textbf{0.4035}^{*}$ & $\textbf{0.7787}^{*}$ & $\textbf{0.2509}$ & $\textbf{0.8937}^{*}$ & $\textbf{0.9093}^{*}$ & $\textbf{0.6960}^{*}$ & $\textbf{0.3790}^{*}$ & $\textbf{0.6296}^{*}$ & $\textbf{0.6520}$ & $\textbf{0.9980}$ & $\textbf{1.0585}^{*}$ & $\textbf{0.2475}^{*}$ & $\textbf{0.5233}^{*}$ \\ 

% \specialrule{0.1em}{1pt}{1pt}
% \end{tabular}}
% \label{tab:main_result}}
% \end{table*}

\begin{table*}[!htbp]
\caption{Results on two public datasets.}
\vspace{-10pt}
\label{tab:main_result}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cccc}
\hline
    Dataset & \multicolumn{6}{c|}{KuaiRand} & \multicolumn{8}{c}{Kaggle-Revenue}  \\
\hline
    {Task} & \multicolumn{2}{c|}{click} & \multicolumn{2}{c|}{long view} & \multicolumn{2}{c|}{watch time} & \multicolumn{2}{c|}{repurchase 1Y} & \multicolumn{2}{c|}{repurchase 1M}& \multicolumn{4}{c}{repurchase 1M amt} \\
\hline
    Metrics & AUC$\uparrow$ & LogLoss$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & NRMSE$\downarrow$ & NMAE$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & NRMSE$\downarrow$ & NMAE$\downarrow$ & Spearman$\uparrow$ & Gini$\uparrow$ \\ 
\hline
    DNN & 0.7512 & 0.4074 & 0.7698 & 0.2536 & 0.8979 & 0.9553 & 0.6892 & 0.3830 & 0.6255 & 0.6542 & 0.9985 & 1.0902 & 0.2339 & 0.5093 \\ 
    Share Bottom & 0.7399 & 0.4115 & 0.7685 & 0.2543 & 0.8968 & 0.9620 & 0.6568 & 0.3931 & 0.6134 & 0.6606 & 0.9984 & 1.1064 & 0.2340 & 0.5090 \\ 
    MMoE & 0.7379 & 0.4127 & 0.7645 & 0.2566 & 0.8970 & 0.9621 & 0.6696 & 0.3903 & 0.6161 & 0.6593 & 0.9987 & \underline{1.0623} & 0.2357 & 0.5093 \\ 
    PLE & 0.7409 & 0.4110 & 0.7694 & 0.2542 & \underline{0.8963} & 0.9648 & 0.6732 & 0.3885 & 0.6178 & 0.6598 & 0.9988 & 1.0708 & 0.2332 & 0.5136 \\
    AdaTT & 0.7396 & 0.4120 & 0.7683 & 0.2550 & 0.8975 & \underline{0.9508} & 0.6720 & 0.3888 & 0.6187 & 0.6580 & 0.9987 & 1.0969 & \underline{0.2419} & \underline{0.5185} \\ 
    ESMM & 0.7303 & 0.4259 & 0.7540 & 0.2832 & 0.8981 & 0.9605 & 0.6361 & 0.6871 & 0.6046 & 0.7755 & 0.9989 & 1.1981 & 0.2379 & 0.5131 \\ 
    AITM & 0.7391 & 0.4118 & 0.7672 & 0.2552 & 0.8978 & 0.9533 & 0.6728 & 0.3871 & 0.6151 & 0.6579 & \underline{0.9982} & 1.1274 & 0.2204 & 0.5029 \\ 
    MetaBalance & \underline{0.7541} & \underline{0.4065} & \underline{0.7768} & \underline{0.2527} & 0.8967 & 0.9509 & \underline{0.6896} & \underline{0.3825} & \underline{0.6267} & \underline{0.6539} & 0.9985 & 1.1265 & 0.2376 & 0.5100 \\ 
\hline
    HTLNet & $\textbf{0.7574}^{*}$ & $\textbf{0.4035}^{*}$ & $\textbf{0.7787}^{*}$ & $\textbf{0.2509}$ & $\textbf{0.8937}^{*}$ & $\textbf{0.9093}^{*}$ & $\textbf{0.6960}^{*}$ & $\textbf{0.3790}^{*}$ & $\textbf{0.6296}^{*}$ & $\textbf{0.6520}$ & $\textbf{0.9980}$ & $\textbf{1.0585}^{*}$ & $\textbf{0.2475}^{*}$ & $\textbf{0.5233}^{*}$ \\ 
\hline
\end{tabular}
}
\begin{tablenotes}\footnotesize
    \item[*] Here the best and second best results are marked in \textbf{bold} and \underline{underline} fonts, respectively. Each experiment is repeated 10 times for statistical confidence, and $^{*}$ indicates a significance level of $p\leq 0.05$ based on a two-sample t-test between our method and the best baseline.
\end{tablenotes}
\end{table*}

==> tables/table_main_product.tex <==

% \begin{table}[htbp]
% \caption{Results on the product dataset, where the best and second best results are marked in bold and underlined, respectively. Note that $^{*}$ indicates a significance level of $p\leq 0.05$ based on a two-sample t-test between our method and the best baseline.}
% \vspace{-5pt}
% \centering
% \scalebox{1.0}{
% \resizebox{0.45\textwidth}{!}{
% \begin{tabular}{c|cc|cc|cccc}
% \specialrule{0.1em}{3pt}{3pt}
%     {Task} & \multicolumn{2}{c|}{click} & \multicolumn{2}{c|}{convert}& \multicolumn{4}{c}{purchase amt} \\
    
%     Metrics & AUC$\uparrow$ & LogLoss$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & NRMSE$\downarrow$ & NMAE$\downarrow$ & Spearman$\uparrow$ & Gini$\uparrow$ \\ 
    
%     \specialrule{0.05em}{1pt}{3pt}
    
%         DNN & 0.7914 & 0.1508 & 0.8929 & 0.1105 & 0.8475 & 0.8471 & 0.1759 & 0.7982 \\ 
%         Share Bottom & 0.7968 & 0.1498 & 0.8991 & 0.1062 & 0.8441 & 0.8499 & 0.1779 & 0.8085 \\ 
%         MMoE & 0.7749 & 0.1544 & 0.8770 & 0.1119 & \underline{0.8351} & 0.8846 & 0.2060 & 0.8254 \\ 
%         PLE & 0.7936 & 0.1500 & 0.8983 & 0.1054 & 0.8507 & 0.9276 & \underline{0.2088} & 0.8274 \\ 
%         AdaTT & 0.7958 & 0.1497 & 0.9000 & 0.1040 & 0.8401 & 0.9234 & 0.2014 & \underline{0.8279} \\ 
%         ESMM & 0.7069 & 0.2324 & 0.8378 & 0.1982 & 0.8594 & \underline{0.8469} & 0.1892 & 0.8128 \\ 
%         AITM & \underline{0.8036} & \underline{0.1479} & 0.9003 & \underline{0.1034} & 0.8377 & 0.8807 & 0.1956 & 0.8212 \\ 
%         MetaBalance & 0.7965 & 0.1492 & \underline{0.9008} & 0.1035 & 0.8365 & 0.9094 & 0.1954 & 0.8219 \\ 
%         HTLNet & $\textbf{0.8049}^{*}$ & $\textbf{0.1472}$ & $\textbf{0.9023}$ & $\textbf{0.1030}$ & $\textbf{0.8346}$ & $\textbf{0.8383}^{*}$ & $\textbf{0.2244}^{*}$ & $\textbf{0.8362}^{*}$ \\ 
% \specialrule{0.1em}{1pt}{1pt}
% \end{tabular}}
% \label{tab:main_result_1}}
% \end{table}

\begin{table}[!htbp]
\caption{Results on the product dataset}
\vspace{-10pt}
\label{tab:main_result_1}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|cc|cc|cccc}
\hline
    Task & \multicolumn{2}{c|}{click} & \multicolumn{2}{c|}{convert} & \multicolumn{4}{c}{purchase amt} \\
\hline
    Metrics & AUC$\uparrow$ & LogLoss$\downarrow$ & AUC$\uparrow$ & LogLoss$\downarrow$ & NRMSE$\downarrow$ & NMAE$\downarrow$ & Spearman$\uparrow$ & Gini$\uparrow$ \\ 
\hline
    DNN & 0.7914 & 0.1508 & 0.8929 & 0.1105 & 0.8475 & 0.8471 & 0.1759 & 0.7982 \\ 
    Share Bottom & 0.7968 & 0.1498 & 0.8991 & 0.1062 & 0.8441 & 0.8499 & 0.1779 & 0.8085 \\ 
    MMoE & 0.7749 & 0.1544 & 0.8770 & 0.1119 & \underline{0.8351} & 0.8846 & 0.2060 & 0.8254 \\ 
    PLE & 0.7936 & 0.1500 & 0.8983 & 0.1054 & 0.8507 & 0.9276 & \underline{0.2088} & 0.8274 \\ 
    AdaTT & 0.7958 & 0.1497 & 0.9000 & 0.1040 & 0.8401 & 0.9234 & 0.2014 & \underline{0.8279} \\ 
    ESMM & 0.7069 & 0.2324 & 0.8378 & 0.1982 & 0.8594 & \underline{0.8469} & 0.1892 & 0.8128 \\ 
    AITM & \underline{0.8036} & \underline{0.1479} & 0.9003 & \underline{0.1034} & 0.8377 & 0.8807 & 0.1956 & 0.8212 \\ 
    MetaBalance & 0.7965 & 0.1492 & \underline{0.9008} & 0.1035 & 0.8365 & 0.9094 & 0.1954 & 0.8219 \\ 
\hline
    HTLNet & $\textbf{0.8049}^{*}$ & $\textbf{0.1472}$ & $\textbf{0.9023}$ & $\textbf{0.1030}$ & $\textbf{0.8346}$ & $\textbf{0.8383}^{*}$ & $\textbf{0.2244}^{*}$ & $\textbf{0.8362}^{*}$ \\ 
\hline
\end{tabular}}
\begin{tablenotes}\footnotesize
\item[*] Here the best and second best results are marked in \textbf{bold} and \underline{underline} fonts, respectively. Each experiment is repeated 10 times for statistical confidence, and $^{*}$ indicates a significance level of $p\leq 0.05$ based on a two-sample t-test between our method and the best baseline.
\end{tablenotes}
\end{table}
